Combining Networks using Cherry Picking Sequences

Phylogenetic networks are important for the study of evolution. The number of methods to find such networks is increasing, but most such methods can only reconstruct small networks. To find bigger networks, one can attempt to combine small networks. In this paper, we study the {\sc Network Hybridization} problem, a problem of combining networks into another network with low complexity. We characterize this complexity via a restricted problem, {\sc Tree-child Network Hybridization}, and we present an FPT algorithm to efficiently solve this restricted problem.

==> Tree-childCompatible.tex <==
\todoYuki{Check proof of thm!}
\begin{theorem}\label{thm:TreeChildCompatible}
Let~$N_1,N_2$ be tree-child networks on~$X$.
Let~$(p_{r_1},r_1)$ and~$(p_{r_2},r_2)$ be reticulation edges in~$N_1,N_2$ respectively, such that $desc_{N_1}(r_1) = L_1$ and~$desc_{N_2}(r_2) = L_2$.
If~$desc_{N_1}(p_{r_1}) = desc_{N_2}(p_{r_2}) = L_1\cup L_2$ then~$N_1$ and~$N_2$ are not tree-child compatible.
\end{theorem}
\begin{proof}
If~$L_1$ and~$L_2$ contain only one leaf, say~$L_1 = \{x\}$ and~$L_2 = \{y\}$, then the parents of~$x$ and~$y$ in~$N_1$ are~$r_1$ and~$p_{r_1}$ respectively; in~$N_2$, the parents of~$x$ and~$y$ are~$p_{r_2}$ and~$r_2$ respectively.
Otherwise, there would be additional reticulation edges between the parents of~$x$ and~$y$, which would violate the tree-child property of networks~$N_1$ and / or~$N_2$.
Therefore we have that~$N_1$ contains the reticulated cherry~$(x,y)$ and~$N_2$ contains the reticulated cherry~$(y,x)$.
Then we are done by Lemma~\ref{lem:reticCherryTCCompatible}.
So we can assume that at least one of the two sets~$L_1$ or~$L_2$ contains at least two leaves.
We show that there exists no TCS which reduces the networks~$N_1$ and~$N_2$.

If a TCS reduces~$N_1$ then by definition, it must contain an element that deletes the edge~$p_{r_1}r_1$.
Similarly if a TCS reduces~$N_2$, then it must contain an element that deletes the edge~$p_{r_2}r_2$.
Suppose for a contradiction that there exists a TCS~$S$ which reduces both networks~$N_1$ and~$N_2$.
Let~$S_i, S_j$ correspond to the reticulated cherries of~$S$ which delete the edges~$p_{r_1}r_1, p_{r_2}r_2$ respectively.
Let~$x_k, y_k$ denote the child of~$r_k, p_{r_k}$ in~$N_k$ respectively for~$k=1,2$: here, we let~$y_k$ denote the child of~$p_{r_k}$ that is not~$r_k$. 
By definition,~$x_1, y_1$ are leaves in~$NS_{[:i-1]}$, and~$x_2, y_2$ are leaves in~$NS_{[:j-1]}$.
It follows then that $S_i$ is the reducible pair~$(x_1, y_1)$ in~$N_1$ and~$S_j$ is the reducible pair~$(x_2, y_2)$ in~$N_2$.
In particular,~$x_k$, for~$k=1,2$, must be the first coordinate in both reducible pairs, as~$x_k$ is below a reticulation node.

Without loss of generality, let~$i<j$.
We claim that the leaf label of~$x_1$ in~$N_1S_{[:i-1]}$ and the leaf label of~$y_2$ in~$N_2S_{[:j-1]}$ is the same, and also that the leaf label of~$y_1$ in~$N_1S_{[:i-1]}$ and the leaf label of~$x_2$ in~$N_2S_{[:j-1]}$ is the same.
By assumption,~$desc_{N_1}(r_1) = L_1, desc_{N_2}(r_2) = L_2$, and~$desc_{N_1}(p_{r_1}) = desc_{N_2}(p_{r_2})= L_1\cup L_2$.
This immediately implies that~$x_1 \in L_1$ and~$x_2 \in L_2$.
Note that every leaf in~$L_1\setminus\{x_1\}$ has been `picked' as a first coordinate of some element in~$S_{[:i-1]}$ to obtain~$x_1$ as a leaf child of~$r_1$, and so~$y_1\in L_2$.
Otherwise~$S_{[:i-1]}$ would not be a tree-child sequence.
By a similar argument,~$y_2\in L_1$.

As mentioned before, every leaf in~$L_1\setminus\{x_1\}$ has been `picked' as a first coordinate of some element in~$S_{[:i-1]}$.
This inherently implies that~$y_2$ must be the leaf~$x_1$: otherwise, we would have a reticulated cherry~$(x_2,y_2)$ in~$N_2S_{[:j-1]}$ that we necessarily have to pick by Lemma~\ref{lem:reducingReticCherries}.
But~$y_2$ would have appeared as a first coordinate in an element of~$S_{[:j-1]}$, which would contradict the fact that~$S$ is a tree-child sequence.
Therefore~$y_2 = x_1$; by an analogous argument,~$x_2 = y_1$.
Now, we have that~$S_i = (x_1,y_1)$ and~$S_j = (y_1,x_1)$.
Then clearly,~$S$ is not a tree-child sequence. 
We have our required contradiction.
\end{proof}

% Therefore, we can decide whether a set of tree-child networks are tree-child compatible by finding the leaf-descendant sets of all reticulations and their parents in all networks, and seeing their pairwise comparison (naively takes~$O(|\mathcal{N}|^2|X|^2)$ time, where~$\cal{N}$ denotes the set of input tree-child networks and~$X$ the taxa set.).
%\yuki{toggled, cuz i dont think this is true in particular. This is not an iff statement.}


\begin{lemma}[Move to the left]\label{lem:Move1Left}
Let $\mathcal{N}=\{N_1,\ldots,N_I\}$ be a set of tree-child networks on a common set of leaves, and let $S(a,b)(x,y)S'$ be a TCS for $\mathcal{N}$. Suppose that for each $N\in\mathcal{N}S$ we have either $x$ is not a leaf in $N$, or $(x,y)$ is a reducible pair of $N$, and there is at least one network such that the latter holds. Then there is a TCS for $\mathcal{N}$ starting with $S(x,y)$ of length equal to $S(a,b)(x,y)S'$.
\end{lemma}
\begin{proof}
Suppose $b=x$. Then there must be a network in $\mathcal{N}S$ that has both the reducible pairs $(x,y)$ and $(a,x)$. This can only occur if $a=y$: as $x$ is the first as well as the second element of a reducible pair, it must form a cherry with another leaf, namely the leaf $y$. However, $S(y,x)(x,y)S'$ is not a TCS, which contradicts our assumption that $S(a,b)(x,y)S'$ is a TCS for $\mathcal{N}$.

Hence, for the rest of the proof, we assume $b\neq x$. In this case, $S(x,y)(a,b)S'$ is a TCS.
It remains to prove that it reduces $\mathcal{N}$. This is clear if $\{x,y\}\cap\{a,b\}=\emptyset$. %because new cherries in a network must involve one of the leaves of the previous pair
We still need to check the cases $a=x$ and for $b=y$. 

In the case that $a=x$, and a network has both reducible pairs $(x,b)$ and $(x,y)$, then the network has a reticulation with reticulated cherries $(x,b)$ and $(x,y)$. The order of reducing these pairs obviously does not matter for such networks: both options remove the reticulation edges between the parents of $b$ and $y$, and the parent of $x$. For a network $N$ that only has the reducible pair $(x,y)$ after $S$ (and not $(x,b)$), the network $NS(x,y)(x,b)$ is a subnetwork of $NS(x,b)(x,y)=NS(x,y)$. This means $S(x,y)(x,b)S'$ also reduces $N$ \cite{YukiRemie}. Hence if $a=x$, the sequence $S(x,y)(a,b)S'$ is a TCS for $\mathcal{N}$.

Now suppose $b=y$. Let $N$ be a network that has both reducible pairs $(a,y)$ and $(x,y)$. In this case the parent of $y$ in $N$ is a multifurcation (a tree node of outdegree at least~$3$). Now $NS(a,y)(x,y)$ and $NS(x,y)(a,y)$ are the same, as for both graphs, the difference between it and $NS$ is the removal of the reticulation edges between the parent of $y$ and the parents of $x$ and $a$, or the deletion of the leaves~$x$ and~$a$ (or some combination of the two, depending on the nature of the reducible pair). Hence $S(x,y)(a,b)S'$ reduces $N$. Now if a network in $\mathcal{N}$ only has the reducible pair $(x,y)$ after $S$ (and not $(a,b)$), then by the same argument as before, first reducing $(x,y)$ and then $(a,b)$ gives a subnetwork, and hence $S(x,y)(a,b)S'$ also reduces such networks. Hence if $b=y$, then $S(x,y)(a,b)S'$ reduces $\mathcal{N}$.
\end{proof}
